MBW: Multi-view Bootstrapping in the Wild

Labeling articulated objects in unconstrained settings have a wide variety of applications including entertainment, neuroscience, psychology, ethology, and many fields of medicine. Large offline labeled datasets do not exist for all but the most common articulated object categories (e.g., humans). Hand labeling these landmarks within a video sequence is a laborious task. Learned landmark detectors can help, but can be error-prone when trained from only a few examples. Multi-camera systems that train fine-grained detectors have shown significant promise in detecting such errors, allowing for self-supervised solutions that only need a small percentage of the video sequence to be hand-labeled. The approach, however, is based on calibrated cameras and rigid geometry, making it expensive, difficult to manage, and impractical in real-world scenarios. In this paper, we address these bottlenecks by combining a non-rigid 3D neural prior with deep flow to obtain high-fidelity landmark estimates from videos with only two or three uncalibrated, handheld cameras. With just a few annotations (representing 1-2% of the frames), we are able to produce 2D results comparable to state-of-the-art fully supervised methods, along with 3D reconstructions that are impossible with other existing approaches. Our Multi-view Bootstrapping in the Wild (MBW) approach demonstrates impressive results on standard human datasets, as well as tigers, cheetahs, fish, colobus monkeys, chimpanzees, and flamingos from videos captured casually in a zoo. We release the codebase for MBW as well as this challenging zoo dataset consisting image frames of tail-end distribution categories with their corresponding 2D, 3D labels generated from minimal human intervention.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sec.~\ref{sec: results}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec: limitation}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Not applicable to the best of our knowledge.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA
	\item Did you include complete proofs of all theoretical results?
    \answerNA
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We release the dataset publicly under CC-BY-NC license. The URL to platform where the dataset can be viewed and downloaded by the reviewers:  {\fontfamily{qcr}\selectfont \textcolor{magenta}{https://github.com/mosamdabhi/MBW-Data}}. We will release the code publicly under MIT license upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Datasplits for each experiments are discussed in Sec.~\ref{sec: results}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Although error bars are explicitly not reported, extensive ablation studies over multiple trials are conducted and shown in Appendix Sec.~\ref{appendix: iterations}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Total amount of compute and type of resources used are discussed in Sec.~\ref{sec: results} under ``{Implementation Details''}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creators of benchmark dataset Human3.6Million~\cite{human36m}. We also cite the creators of Recurrent All-pairs Field Transform(RAFT)~\cite{raft}, Multi-View Non-Rigid-Structure-from-Motion (MV-NRSfM)~\cite{dabhi3dv}, and Deep High-Resolution Representation Learning for Human Pose Estimation (HRNet)~\cite{hrnet}.}
  \item Did you mention the license of the assets?
    \answerYes{Although not explicitly mentioned in the text, we mention the license below.}
    \begin{itemize}
        \item Human3.6Million dataset~\cite{human36m} was used under the license of CC-BY-NC.
        \item RAFT~\cite{raft} codebase was used under BSD-3-Clause license.
        \item HRNet~\cite{hrnet} codebase used under MIT license.
        \item MV-NRSfM~\cite{dabhi3dv}: No existing code assets were used.
    \end{itemize}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{
    % \paragraph{Data assets: Fish, Chimpanzee, Colobus Monkey}
    \paragraph{Data assets} We release a zoo dataset (captured by authors) consisting 2-View synchronized video frames, manual 2D landmark annotations (for 1-2\% of frames), predicted 2D and 3D landmark annotations for each instance, confidence flag associated with each instance specifying how much we should rely on the generated prediction (calculated using Eq.~\eqref{eq:uncertainty_score}, and finally bounding box information for each instance.}
    
    % \paragraph{Data asset: Tiger, Clownfish, Seahorse data asset} We also release a Tiger, Clownfish, and Seahorse dataset consisting 2-View synchronized video frames, and manual 2D landmark annotations (for 1-2\% of frames).}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Although not discussed within the text, we confirm that no personally identifiable information or offensive content exists in the released data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

